Comprehension Based Question Answering using Bloom's Taxonomy

Current pre-trained language models have lots of knowledge, but a more limited ability to use that knowledge. Bloom's Taxonomy helps educators teach children how to use knowledge by categorizing comprehension skills, so we use it to analyze and improve the comprehension skills of large pre-trained language models. Our experiments focus on zero-shot question answering, using the taxonomy to provide proximal context that helps the model answer questions by being relevant to those questions. We show targeting context in this manner improves performance across 4 popular common sense question answer datasets.

==> dataset.tex <==
\section{Dataset}
% We evaluate ou

% We evaluate our study on 6 \mc{We just want the 4 datasets where we get differentiation across clarification level, right? (The ones mentioned in \tabref{table:prefixes}.} different types of multiple question answering tasks: COPA(Gordon et al., 2012), CommonSenseQA (Talmor et al., 2019), MC-TACO (Zhou et al., 2019), Social IQa (Sap et al., 2019b), PIQA (Bisk et al., 2020), WinoGrande (Sakaguchi et al., 2020).

% COPA is a commonsense causal reasoning dataset, where each question is comprised of a premise and two candidate hypotheses. The task is to pick the correct hypothesis that better fits the causal relation with the premise.

% Social IQA is another dataset to benchmark commonsense question answering task. It measures the reasoning about actions and social dynamics underlying the situation described in the context. The task is predict the best possible choice that explains the social implication out of three alternatives.

% Winogrande is a collection of WSC challenge problems crowdsourced through MTurk. The data present is less biased as it was processed with an adversarial filtering algorithm.
